Novel Knockoff Generation and Importance Measures with Heterogeneous Data via Conditional Residuals and Local Gradients

Knockoff variable selection is a powerful framework that creates synthetic knockoff variables to mirror the correlation structure of the observed features, enabling principled control of the false discovery rate in variable selection. However, existing methods often assume homogeneous data types or known distributions, limiting their applicability in real-world settings with heterogeneous, distribution-free data. Moreover, common variable importance measures rely on linear outcome models, hindering their effectiveness for complex relationships. We propose a flexible knockoff generation framework based on conditional residuals that accommodates mixed data types without assuming known distributions. To assess variable importance, we introduce the Mean Absolute Local Derivative (MALD), an interpretable metric compatible with nonlinear outcome functions, including random forests and neural networks. Simulations show that our approach achieves better false discovery rate control and higher power than existing methods. We demonstrate its practical utility on a DNA methylation dataset from mouse tissues, identifying CpG sites linked to aging. Software is available in R (rangerKnockoff) and Python (MALDimportance).

==> SpecialCharacters.tex <==
% ===============================================================
% special characters
% ===============================================================
\newcommand{\rd}[1]{\textcolor{red}{#1}}

\def\wt{\widetilde}
\def\diag{\hbox{diag}}
\def\wh{\widehat}
\def\wb{\overline}
\def\AIC{\hbox{AIC}}
\def\BIC{\hbox{BIC}}


\newcommand{\beq}{\begin{equation}}
	\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
	\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beas}{\begin{eqnarray*}}
	\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\pari}{\hspace{\parindent}}
\newcommand{\nn}{\nonumber}
\newcommand{\myupvspace}{-\myht}
\newcommand{\mydnvspace}{.3in}
\newcommand{\mybotvspace}{.1in}
\newcommand{\mywid}{2.3in}
\newcommand{\mywidw}{1.8in}
\newcommand{\myht}{1.8in}
\newcommand{\myhspace}{2.5in}
\newcommand{\mydhspace}{5in}
\newcommand{\bct}{\begin{center}}
	\newcommand{\ect}{\end{center}}
\newcommand{\gf}{\includegraphics}


%%\newtheorem{theorem}{Theorem}[section]
%% \newtheorem{theorem}{Theorem}
\newtheorem{acknowledgement}[theorem]{Acknowledgement}
% \newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{axiom}[theorem]{Axiom}
\newtheorem{case}[theorem]{Case}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{criterion}[theorem]{Criterion}
\newtheorem{definition}{Definition}
%\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{remark}[theorem]{Remark}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{summary}[theorem]{Summary}

\iffalse
\newenvironment{proof}[1][Proof]{\begin{trivlist}
		\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}


\newcommand{\qed}{\nobreak \ifvmode \relax \else
	\ifdim\lastskip<1.5em \hskip-\lastskip
	\hskip1.5em plus0em minus0.5em \fi \nobreak
	\vrule height0.75em width0.5em depth0.25em\fi}
        
\fi

\newcommand{\ts}{\textsuperscript}
\newcommand{\sis}{\sigma^2}
\newcommand{\ba}{ {\bf a} }
\newcommand{\bA}{ {\bf A} }
\newcommand{\bb}{ {\bf b} }
\newcommand{\bB}{ {\bf B} }
\newcommand{\bc}{ {\bf c} }
\newcommand{\bC}{ {\bf C} }
\newcommand{\bd}{ {\bf d} }
\newcommand{\bD}{ {\bf D} }
\newcommand{\be}{ {\bf e} }
\newcommand{\bE}{ {\bf E} }
\newcommand{\boldf}{ {\bf f} }
\newcommand{\bF}{ {\bf F} }
\newcommand{\bg}{ {\bf g} }
\newcommand{\bG}{ {\bf G} }
\newcommand{\bh}{ {\bf h} }
\newcommand{\bH}{ {\bf H} }
\newcommand{\bi}{ {\bf i} }
\newcommand{\bI}{ {\bf I} }
\newcommand{\bj}{ {\bf j} }
\newcommand{\bJ}{ {\bf J} }
\newcommand{\bk}{ {\bf k} }
\newcommand{\bK}{ {\bf K} }
\newcommand{\bl}{ {\bf l} }
\newcommand{\bL}{ {\bf L} }
% \newcommand{\bm}{ {\bf m} }
\newcommand{\bM}{ {\bf M} }
\newcommand{\bn}{ {\bf n} }
\newcommand{\bN}{ {\bf N} }
\newcommand{\bo}{ {\bf o} }
\newcommand{\bO}{ {\bf O} }
\newcommand{\bp}{ {\bf p} }
\newcommand{\bP}{ {\bf P} }
\newcommand{\bq}{ {\bf q} }
\newcommand{\bQ}{ {\bf Q} }
\newcommand{\br}{ {\bf r} }
\newcommand{\bR}{ {\bf R} }
\newcommand{\bs}{ {\bf s} }
\newcommand{\bS}{ {\bf S} }
\newcommand{\bt}{ {\bf t} }
\newcommand{\bT}{ {\bf T} }
\newcommand{\bu}{ {\bf u} }
\newcommand{\bU}{ {\bf U} }
\newcommand{\bv}{ {\bf v} }
\newcommand{\bV}{ {\bf V} }
\newcommand{\bw}{ {\bf w} }
\newcommand{\bW}{ {\bf W} }
\newcommand{\bx}{ {\bf x} }
\newcommand{\bX}{ {\bf X} }
\newcommand{\by}{ {\bf y} }
\newcommand{\bY}{ {\bf Y} }
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bZ}{\mathbf{Z}}


\def\bbR{\mathbb{R}}
\def\bbN{\mathbb{N}}


\newcommand{\MX}{{\mathbb X}}
\newcommand{\MY}{{\mathbb Y}}
\newcommand{\MZ}{{\mathbb Z}}
\newcommand{\MU}{{\mathbb U}}
\newcommand{\MR}{{\mathbb R}}
\newcommand{\MS}{{\mathbb S}}
\newcommand{\MO}{{\mathbb O}}
\newcommand{\MP}{{\mathbb P}}
\newcommand{\MQ}{{\mathbb Q}}
\newcommand{\MPsi}{{\mathbb \Psi}}


\newcommand{\balph}{ {\boldsymbol \alpha} }
\newcommand{\balpha}{ {\boldsymbol \alpha} }
\newcommand{\bbet}{ {\boldsymbol \beta} }
\newcommand{\bbeta}{ {\boldsymbol \beta} }
\newcommand{\bgam}{ {\boldsymbol \gamma} }
\newcommand{\bgamma}{ {\boldsymbol \gamma} }
\newcommand{\bGamma}{ {\boldsymbol \Gamma} }
\newcommand{\bdelta}{ {\boldsymbol \delta} }
\newcommand{\bDelta}{ {\boldsymbol \Delta} }
\newcommand{\beps}{ {\boldsymbol \epsilon} }
\newcommand{\bepsilon}{ {\boldsymbol \epsilon} }
\newcommand{\bphi}{ {\boldsymbol \phi} }
\newcommand{\bPhi}{ {\boldsymbol \Phi} }
\newcommand{\bpi}{ {\boldsymbol \pi} }
\newcommand{\bnu}{ {\boldsymbol \nu} }
\newcommand{\bkap}{ {\boldsymbol \kappa} }
\newcommand{\bkappa}{ {\boldsymbol \kappa} }
\newcommand{\bKappa}{ {\boldsymbol \Kappa} }
\newcommand{\blam}{ {\boldsymbol \lambda} }
\newcommand{\blambda}{ {\boldsymbol \lambda} }
\newcommand{\bLambda}{ {\boldsymbol \Lambda} }
\newcommand{\bmu}{ {\boldsymbol \mu} }
\newcommand{\bMu}{ {\boldsymbol \Mu} }
\newcommand{\bet}{ {\boldsymbol \eta} }
\newcommand{\bome}{ {\boldsymbol \omega} }
\newcommand{\bomega}{ {\boldsymbol \omega} }
\newcommand{\bOmega}{ {\boldsymbol \Omega} }
\newcommand{\bnabla}{ {\boldsymbol \nabla} }
\newcommand{\brho}{ {\boldsymbol \rho} }
\newcommand{\bsigma}{ {\boldsymbol \sigma} }
\newcommand{\bSig}{ {\boldsymbol \Sigma} }
\newcommand{\bSigma}{ {\boldsymbol \Sigma} }
\newcommand{\btheta}{ {\boldsymbol \theta} }
\newcommand{\bTheta}{ {\boldsymbol \Theta} }
\newcommand{\bzeta}{ {\boldsymbol \zeta} }
\newcommand{\bPsi}{ {\boldsymbol \Psi} }

\newcommand{\bzero}{ {\boldsymbol 0} }
\newcommand{\bones}{ {\boldsymbol 1} }

\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother


\def\olbx{\overline{\bx}}
\def\bzero{\mathbf{0}}
\def\bone{\mathbf{1}}
\def\argmin{\operatornamewithlimits{argmin}}
\def\argmax{\operatornamewithlimits{argmax}}
\def\bbeta{\boldsymbol{\beta}}
\def\bb{\mathbf{b}}
\def\bB{\mathbf{B}}
\def\bc{\mathbf{c}}
\def\RF{\mathrm{RF}}
\def\tr{\mathrm{tr}}
\def\cov{\mathrm{Cov}}
\def\diag{\operatorname{diag}}
\def\bdelta{\boldsymbol{\delta}}
\def\bD{\mathbf{D}}
\def\bd{\mathbf{d}}
\def\bDelta{\boldsymbol{\Delta}}
\def\bepsilon{\boldsymbol{\epsilon}}
\def\boldeta{\boldsymbol{\eta}}
\def\E{\mathrm{E}}
\def\bgamma{\boldsymbol{\gamma}}
\def\bGamma{\boldsymbol{\Gamma}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bI{\mathbf{I}}
\def\rI{\mathrm{I}}
\def\rpv{\mathrm{pv}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\logit{\mathrm{logit}}
\def\bkappa{\boldsymbol{\kappa}}
\def\bOmega{\boldsymbol{\Omega}}
\def\pr{\mathrm{P}}
\def\bphi{\boldsymbol{\phi}}
\def\bpsi{\boldsymbol{\psi}}
\def\brho{\boldsymbol{\rho}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\sign{\mathrm{sign}}
\def\bsigma{\boldsymbol{\sigma}}
\def\bSigma{\boldsymbol{\Sigma}}
\def\btau{\boldsymbol{\tau}}
\def\btheta{\boldsymbol{\theta}}
\def\bS{\mathbf{S}}
\def\bs{\mathbf{s}}
\def\bT{\mathbf{T}}
\def\bx{\mathbf{x}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bU{\mathbf{U}}
\def\var{\mathrm{Var\,}}
\def\bV{\mathbf{V}}
\def\bxi{\boldsymbol{\xi}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bE{\mathbf{E\,}}
\def\be{\mathbf{e}}
\def\bF{\mathbf{F}}
\def\bg{\mathbf{g}}
\def\bfG{\mathbf{G}}
\def\bfphi{\boldsymbol\phi}
\def\mo{\mathrm{o}}
\def\FDR{\mathrm{FDR}}
\def\TE{\mathrm{TE}}
\def\IE{\mathrm{IE}}
\def\DE{\mathrm{DE}}
\def\all{\mathrm{all}}
\def\bfg{\mathbf g}


\newcommand{\given}{\,|\,}

\newcommand{\tildeC}{\tilde{C}}
\newcommand{\tildeK}{\tilde{K}}
\newcommand{\tildew}{\tilde{w}}
\newcommand{\tildebw}{\tilde{\bw}}
\newcommand{\tildebW}{\tilde{\bW}}
\newcommand{\tildeeps}{\tilde{\epsilon}}

\newcommand{\eps}{ {\epsilon} }
\newcommand{\boeta}{ \mbox{\boldmath $\eta$} }

\newcommand{\deq}{\stackrel{\mathrm{d}}{=}}

\newcommand{\iid}{\stackrel{\mathrm{iid}}{\sim}}
\newcommand{\tildebC}{\tilde{\bC}}


\def\cM{\mathcal{M}}
\def\cF{\mathcal{F}}
\def\cI{\mathcal{I}}
\def\cZ{\mathcal{Z}}
\def\cY{\mathcal{Y}}
\def\cG{\mathcal{G}}
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\rT{\mathrm{T}}
\def\rS{\mathrm{S}}
\def\rs{\mathrm{s}}


\newcommand{\cE}{{\cal E}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\tp}{{\tilde p}}
\newcommand{\nt}{{N_\theta}}

% \newcommand{\var}{\mathsf{var}}
% \newcommand{\cov}{\mathsf{cov}}
% \newcommand{\diag}{\mbox{diag}}
\newcommand{\taus}{\tau^2}
\newcommand{\sigs}{\sigma^2}

\newcommand{\T}{\top}




==> macros.tex <==
%%-------------------macros definition-------------------------%%
% \newtheorem{lemma}{{Lemma}}
% \newtheorem{assumption}{{ Assumption}}
\newtheorem{theorem}{{Theorem}}
% \newtheorem{corollary}{{Corollary}}
% \newtheorem{definition}{{Definition}}
% \newtheorem{proposition}{{Proposition}}
\newcommand{\HRule}{\rule{\linewidth}{0.5mm}}


\usepackage{amsmath}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\prox}{prox}

\def\tran{^{\mathsf{T}}}
\def\invtran{^{\mathsf{-T}}}
\def\one{\mathds{1}}
\def\hr{\noindent \\\hrule}
\def\sgn{{\rm sgn}}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


% \DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\bp}{ \begin{proof}}
        %\newcommand{\bp}{\footnotesize \begin{proof}}
        \newcommand{\ep}{\end{proof} }

% \newtheorem{remark}[theorem]{Remark}


% ===============================================================
% special characters
% ===============================================================

\newcommand{\rd}[1]{\textcolor{red}{#1}}

\def\wt{\widetilde}
\def\diag{\hbox{diag}}
\def\wh{\widehat}
\def\wb{\overline}
\def\AIC{\hbox{AIC}}
\def\BIC{\hbox{BIC}}



\def\olbx{{\overline{\bx}}}
\def\b0{\mathbf{0}}
\def\b1{\mathbf{1}}
\def\balpha{{\boldsymbol{\alpha}}}
%\def\argmin{\operatornamewithlimits{argmin}}
%\def\argmax{\operatornamewithlimits{argmax}}
\def\bA{\mathbf{A}}
\def\bbeta{{\boldsymbol{\beta}}}
\def\bb{\mathbf{b}}
\def\bz{\mathbf{z}}
\def\bB{\mathbf{B}}
\def\bc{\mathbf{c}}
\def\cov{\mathrm{Cov}}
\def\diag{\operatorname{diag}}
\def\bdelta{{\boldsymbol{\delta}}}
\def\bD{\mathbf{D}}
\def\bd{\mathbf{d}}
\def\bDelta{{\boldsymbol{\Delta}}}
\def\bepsilon{{\boldsymbol{\epsilon}}}
\def\boldeta{{\boldsymbol{\eta}}}
\def\E{\mathrm{E}}
\def\bgamma{{\boldsymbol{\gamma}}}
\def\bGamma{{\boldsymbol{\Gamma}}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bI{\mathbf{I}}
\def\rI{\mathrm{I}}
\def\rpv{\mathrm{pv}}


\def\bC{\mathbf{C}}
\def\bA{\mathbf{A}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bZ{\mathbf{Z}}
\def\logit{\mathrm{logit}}
\def\bmu{{\boldsymbol{\mu}}}
\def\bkappa{{\boldsymbol{\kappa}}}
\def\bOmega{{\boldsymbol{\Omega}}}
\def\pr{\mathrm{P}}
\def\bphi{{\boldsymbol{\phi}}}
\def\bpsi{{\boldsymbol{\psi}}}
\def\brho{{\boldsymbol{\rho}}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\sign{\mathrm{sign}}
\def\bsigma{{\boldsymbol{\sigma}}}
\def\bSigma{{\boldsymbol{\Sigma}}}
\def\btau{{\boldsymbol{\tau}}}
\def\btheta{{\boldsymbol{\theta}}}
\def\bS{\mathbf{S}}
\def\bs{\mathbf{s}}
\def\bT{\mathbf{T}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bU{\mathbf{U}}
\def\var{\mathrm{Var\,}}
\def\bV{\mathbf{V}}
\def\bxi{{\boldsymbol{\xi}}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\by{\mathbf{y}}
\def\bE{\mathbf{E\,}}
% \def\be{\mathbf{e}}
\def\bF{\mathbf{F}}
\def\bg{\mathbf{g}}
\def\bfG{\mathbf{G}}
\def\bfphi{{\boldsymbol\phi}}
\def\mo{\mathrm{o}}
\def\TE{\mathrm{TE}}
\def\IE{\mathrm{IE}}
\def\DE{\mathrm{DE}}
\def\all{\mathrm{all}}
\def\bfg{\mathbf g}
\def\bbR{\mathbb{R}}

\def\rT{\mathrm{T}}
\def\rS{\mathrm{S}}
\def\rs{\mathrm{s}}


\newcommand{\Ex}{{E}\hspace{0.05cm}}
\newcommand{\Exf}{\mathbb{E}_{\mathcal{F}_{i}}\hspace{0.05cm}}
\newcommand{\Exfp}{\mathbb{E}_{\mathcal{F}_{i-1}}\hspace{0.05cm}}
\newcommand{\bm}[1]{\mbox{\boldmath $#1$}}
\newcommand{\no}{\noindent}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bqq}{\begin{eqnarray}}
\newcommand{\eqq}{\end{eqnarray}}
\newcommand{\bal}{\begin{align}}
\newcommand{\eal}{\end{align}}
\newcommand{\bqn}{\begin{eqnarray*}}
        \newcommand{\eqn}{\end{eqnarray*}}
\newcommand{\nn}{\nonumber}
\newcommand{\ba}{\left[ \begin{array}]}
        \newcommand{\ea}{\\ \end{array} \right]}
\newcommand{\qd}{\hfill{$\blacksquare$}}
\newcommand{\define}{\;\stackrel{\Delta}{=}\;}
\newcommand{\aseq}{\;\stackrel{a.s.}{=}\;}
\newcommand{\Tr}{\mbox{\rm {\small Tr}}}

\def\btheta  {{\boldsymbol \theta}}
\def\bxi        {{\boldsymbol \xi}}
\def\bmu        {{\boldsymbol \mu}}
\def\bpsi       {{\boldsymbol \psi}}
\def\bsigma  {{\boldsymbol \sigma}}
\def\bphi  {{\boldsymbol \phi}}
\def\blambda {{\boldsymbol \lambda}}
\def\bTheta  {{\boldsymbol \Theta}}
\def\bSigma  {{\boldsymbol \Sigma}}
\def\bLambda {{\boldsymbol \Lambda}}
\def\bgamma {{\boldsymbol \gamma}}
\def\bepsilon {{\boldsymbol \epsilon}}
\def\Pr {{\mathbb{P}}}
\def\vec {{{\rm vec}}}
\def\tphi   {\widetilde{\boldsymbol \phi}}

\def\A{{\boldsymbol{A}}}
\def\B{{\boldsymbol{B}}}
\def\C{{\boldsymbol{C}}}
\def\D{{\boldsymbol{D}}}
\def\E{{\boldsymbol{E}}}
\def\F{{\boldsymbol{F}}}
\def\G{{\boldsymbol{G}}}
\def\H{{\boldsymbol{H}}}
\def\I{{\boldsymbol{I}}}
\def\J{{\boldsymbol{J}}}
\def\K{{\boldsymbol{K}}}
\def\L{{\boldsymbol{L}}}
\def\M{{\boldsymbol{M}}}
\def\N{{\boldsymbol{N}}}
\def\O{{\boldsymbol{O}}}
\def\P{{\boldsymbol{P}}}
\def\Q{{\boldsymbol{Q}}}
\def\R{{\boldsymbol{R}}}
\def\S{{\boldsymbol{S}}}
\def\T{{\boldsymbol{T}}}
\def\U{{\boldsymbol{U}}}
\def\V{{\boldsymbol{V}}}
\def\W{{\boldsymbol{M}}}
\def\X{{\boldsymbol{X}}}
\def\Y{{\boldsymbol{Y}}}
\def\Z{{\boldsymbol{Z}}}


\def\a{{\boldsymbol{a}}}
\def\b{{\boldsymbol{b}}}
\def\c{{\boldsymbol{c}}}
\def\d{{\boldsymbol{d}}}
\def\e{{\boldsymbol{e}}}
\def\f{{\boldsymbol{f}}}
\def\g{{\boldsymbol{g}}}
\def\h{{\boldsymbol{h}}}
\def\i{{\boldsymbol{i}}}
\def\j{{\boldsymbol{j}}}
\def\k{{\boldsymbol{k}}}
\def\l{{\boldsymbol{l}}}
\def\m{{\boldsymbol{m}}}
\def\n{{\boldsymbol{n}}}
\def\o{{\boldsymbol{o}}}
\def\p{{\boldsymbol{p}}}
\def\q{{\boldsymbol{q}}}
\def\r{{\boldsymbol{r}}}
\def\s{{\boldsymbol{s}}}
\def\t{{\boldsymbol{t}}}
\def\u{{\boldsymbol{u}}}
\def\v{{\boldsymbol{v}}}
\def\w{{\boldsymbol{w}}}
\def\x{{\boldsymbol{x}}}
\def\y{{\boldsymbol{y}}}
\def\z{{\boldsymbol{z}}}

\newcommand{\va}{{\mathbf{a}}}
\newcommand{\vb}{{\mathbf{b}}}
\newcommand{\vc}{{\mathbf{c}}}
\newcommand{\vd}{{\mathbf{d}}}
\newcommand{\ve}{{\mathbf{e}}}
\newcommand{\vf}{{\mathbf{f}}}
\newcommand{\vg}{{\mathbf{g}}}
\newcommand{\vh}{{\mathbf{h}}}
\newcommand{\vi}{{\mathbf{i}}}
\newcommand{\vj}{{\mathbf{j}}}
\newcommand{\vk}{{\mathbf{k}}}
\newcommand{\vl}{{\mathbf{l}}}
\newcommand{\vm}{{\mathbf{m}}}
\newcommand{\vn}{{\mathbf{n}}}
\newcommand{\vo}{{\mathbf{o}}}
\newcommand{\vp}{{\mathbf{p}}}
\newcommand{\vq}{{\mathbf{q}}}
\newcommand{\vr}{{\mathbf{r}}}
\newcommand{\vs}{{\mathbf{s}}}
\newcommand{\vt}{{\mathbf{t}}}
\newcommand{\vu}{{\mathbf{u}}}
%\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\vw}{{\mathbf{w}}}
\newcommand{\vx}{{\mathbf{x}}}
\newcommand{\vy}{{\mathbf{y}}}
\newcommand{\vz}{{\mathbf{z}}}

\newcommand{\vA}{{\mathbf{A}}}
\newcommand{\vB}{{\mathbf{B}}}
\newcommand{\vC}{{\mathbf{C}}}
\newcommand{\vD}{{\mathbf{D}}}
\newcommand{\vE}{{\mathbf{E}}}
\newcommand{\vF}{{\mathbf{F}}}
\newcommand{\vG}{{\mathbf{G}}}
\newcommand{\vH}{{\mathbf{H}}}
\newcommand{\vI}{{\mathbf{I}}}
\newcommand{\vJ}{{\mathbf{J}}}
\newcommand{\vK}{{\mathbf{K}}}
\newcommand{\vL}{{\mathbf{L}}}
\newcommand{\vM}{{\mathbf{M}}}
\newcommand{\vN}{{\mathbf{N}}}
\newcommand{\vO}{{\mathbf{O}}}
\newcommand{\vP}{{\mathbf{P}}}
\newcommand{\vQ}{{\mathbf{Q}}}
\newcommand{\vR}{{\mathbf{R}}}
\newcommand{\vS}{{\mathbf{S}}}
\newcommand{\vT}{{\mathbf{T}}}
\newcommand{\vU}{{\mathbf{U}}}
\newcommand{\vV}{{\mathbf{V}}}
\newcommand{\vW}{{\mathbf{W}}}
\newcommand{\vX}{{\mathbf{X}}}
\newcommand{\vY}{{\mathbf{Y}}}
\newcommand{\vZ}{{\mathbf{Z}}}


\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cZ}{{\mathcal{Z}}}

\newcommand{\tA}{{\widetilde{A}}}
\newcommand{\tB}{{\widetilde{B}}}
\newcommand{\tC}{{\widetilde{C}}}
\newcommand{\tD}{{\widetilde{D}}}
\newcommand{\tE}{{\widetilde{E}}}
\newcommand{\tF}{{\widetilde{F}}}
\newcommand{\tG}{{\widetilde{G}}}
\newcommand{\tH}{{\widetilde{H}}}
\newcommand{\tI}{{\widetilde{I}}}
\newcommand{\tJ}{{\widetilde{J}}}
\newcommand{\tK}{{\widetilde{K}}}
\newcommand{\tL}{{\widetilde{L}}}
\newcommand{\tM}{{\widetilde{M}}}
\newcommand{\tN}{{\widetilde{N}}}
\newcommand{\tO}{{\widetilde{O}}}
\newcommand{\tP}{{\widetilde{P}}}
\newcommand{\tQ}{{\widetilde{Q}}}
\newcommand{\tR}{{\widetilde{R}}}
\newcommand{\tS}{{\widetilde{S}}}
\newcommand{\tT}{{\widetilde{T}}}
\newcommand{\tU}{{\widetilde{U}}}
\newcommand{\tV}{{\widetilde{V}}}
\newcommand{\tW}{{\widetilde{W}}}
\newcommand{\tX}{{\widetilde{X}}}
\newcommand{\tY}{{\widetilde{Y}}}
\newcommand{\tZ}{{\widetilde{Z}}}

\newcommand{\scp}{\boldsymbol{\scriptstyle{\mathcal{P}}}}
\newcommand{\sr}{{\scriptstyle{\mathcal{R}}}}
\newcommand{\su}{\boldsymbol{\scriptstyle{\mathcal{U}}}}
\newcommand{\sv}{\boldsymbol{\scriptstyle{\mathcal{V}}}}
\newcommand{\sw}{\boldsymbol{\scriptstyle{\mathcal{W}}}}
\newcommand{\sx}{\boldsymbol{\scriptstyle{\mathcal{X}}}}
\newcommand{\sz}{\boldsymbol{\scriptstyle{\mathcal{Z}}}}
\newcommand{\sxb}{\boldsymbol{\scriptstyle{\mathcal{X}}}}
\newcommand{\tw}{\widetilde{\boldsymbol{w}}}



% === Kun's Notation ===
\newcommand{\swb}{{\boldsymbol{\scriptstyle{\mathcal{W}}}}}
\newcommand{\barA}{\overline{A}}
\newcommand{\grad}{{\nabla}}
\newcommand{\emp}{{\mathrm{emp}}}
\newcommand{\mb}{{\mathrm{mb}}}
\def\bE{\mathbb{E}}
\def\filt{\boldsymbol{\mathcal{F}}}
\def\ntran{^{-\mathsf{T}}}

\newcommand{\eq}[1]{\begin{align}#1\end{align}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\defeq}{{\stackrel{\triangle}{=}}}
%\newtheorem{remark}{Remark}
\newcommand{\nnb}{\nonumber \\}
\newcommand{\dom}{{\mathrm{dom}}} % domain
\newcommand{\RR}{\mathbb{R}}



\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
        <5> <6> <7> <8> <9> <10>
        <10.95> <12> <14.4> <17.28> <20.74> <24.88>
        mathx10
}{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareFontSubstitution{U}{mathx}{m}{n}
% \DeclareMathAccent{\widebar}{0}{mathx}{"73}


% === Personal settings below ===
\newcommand{\vzero}{\mathbf{0}}
\newcommand{\vone}{{\mathbf{1}}}

%\DeclareMathOperator*{\argmin}{argmin}
%\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\Min}{minimize}
%\DeclareMathOperator*{\Max}{maximize}

%\DeclareMathOperator{\St}{{subject~to}} % subject to

% === Code style settings ===
\usepackage[utf8]{inputenc}

\usepackage{listings}
\usepackage{xcolor}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}

\lstset{style=mystyle}

